Neural Learning of One-of-Many Solutions for Combinatorial Problems in Structured Output Spaces

Recent research has proposed neural architectures for solving combinatorial problems in structured output spaces. In many such problems, there may exist multiple solutions for a given input, e.g. a partially filled Sudoku puzzle may have many completions satisfying all constraints. Further, we are often interested in finding any one of the possible solutions, without any preference between them. Existing approaches completely ignore this solution multiplicity. In this paper, we argue that being oblivious to the presence of multiple solutions can severely hamper their training ability. Our contribution is two fold. First, we formally define the task of learning one-of-many solutions for combinatorial problems in structured output spaces, which is applicable for solving several problems of interest such as N-Queens, and Sudoku. Second, we present a generic learning framework that adapts an existing prediction network for a combinatorial problem to handle solution multiplicity. Our framework uses a selection module, whose goal is to dynamically determine, for every input, the solution that is most effective for training the network parameters in any given learning iteration. We propose an RL based approach to jointly train the selection module with the prediction network. Experiments on three different domains, and using two different prediction networks, demonstrate that our framework significantly improves the accuracy in our setting, obtaining up to 21 pt gain over the baselines.

==> background.tex <==
\section{Background}
\vspace{-1ex}
\label{sec:background}
\textbf{Neural Architectures for Symbolic Reasoning:
}
Recently many neural architectures have been proposed for symbolic and relational reasoning tasks. 
They inductively learn the underlying constraints or relationships between the symbols from input output pairs. 
For example, \cite{dong&al19} propose Neural Logic Machines (NLM) which realizes Horn Clauses \cite{horn51} in First Order Logic (FOL). 
It sequentially applies first order rules on a set of given predicates grounded on a set of objects and learns new predicates in terms of the given ones. 
Predicates are internally represented as tensors and logical operations on predicates are approximated via MLPs on their groundings. 
In NLM, since the invariants are predicates and not their groundings, it is able to learn lifted rules which can transfer over different instance sizes of the same problem. \eg\ NLM can transfer rules learned for N-Queens on $N \times N$ chess board to (N+1)-Queens problem on $(N+1) \times (N+1)$ chess board.

\cite{palm&al18} propose Recurrent Relational Networks (RRN) which use a graph neural network to learn relationships between symbols represented as nodes of the graph. 
It can be used for any task that requires multi-step relational reasoning, \eg\ solving Sudoku.
However, unlike NLM, the symbols are tied to the network architecture and hence it can not generalize across problem size, \ie\ one cannot solve $4 \times 4$ Sudoku using an RRN trained on $9 \times 9$ grid.

\cite{wang&al19} propose a differentiable maximum satisfiability (MAXSAT) solver by representing the MAXSAT problem as a low rank Semi Definite Program (SDP). 
Given a partial assignment of variables (or universe?), it assigns value to remaining boolean variables according to the MAXSAT problem it learns to represent.
Similar to RRN, it cannot generalize across size as the matrix representing an SDP is tied to the symbols of the underlying problem.  
\dcom{Is SATNet description needed?}

